InterroLang: Exploring NLP Models and Datasets through Dialogue-based Explanations

While recently developed NLP explainability methods let us open the black box in various ways (Madsen et al., 2022), a missing ingredient in this endeavor is an interactive tool offering a conversational interface. Such a dialogue system can help users explore datasets and models with explanations in a contextualized manner, e.g. via clarification or follow-up questions, and through a natural language interface. We adapt the conversational explanation framework TalkToModel (Slack et al., 2022) to the NLP domain, add new NLP-specific operations such as free-text rationalization, and illustrate its generalizability on three NLP tasks (dialogue act classification, question answering, hate speech detection). To recognize user queries for explanations, we evaluate fine-tuned and few-shot prompting models and implement a novel Adapter-based approach. We then conduct two user studies on (1) the perceived correctness and helpfulness of the dialogues, and (2) the simulatability, i.e. how objectively helpful dialogical explanations are for humans in figuring out the model's predicted label when it's not shown. We found rationalization and feature attribution were helpful in explaining the model behavior. Moreover, users could more reliably predict the model outcome based on an explanation dialogue rather than one-off explanations.

==> tables/describing_feature_importance.tex <==
\section{Describing feature importance}
\label{app:featureimportance}

\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
    \item Part-of-speech information: The adjective/noun/... is salient
    \item Entity information: The location/person/... is salient
    \item Syntactic vs. semantic information: The wh-words/function words/punctuations/... are salient
    \item Span description: The NP/VP/dependency head/... is salient
    \item Position in text: The first/last sentence contains the most salient token $x$. / Token $x$ is located between tokens $y$ and $z$.
    \item Sentence type: The question/longest sentence/... contains the most salient token(s)
    \item Entailment relation: The salient $x$ entails/contradicts $y$
    \item Semantic similarity: The salient $x$ is similar/related to $y$ (retrieve similar words for contextualization)
    \item WordNet relations: $x$ is a hypernym/hyponym of $y$
\end{itemize}

In addition, we can contextualize the saliency information like such:
\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
    \item Relation between local and global salience: $x$ is more salient for this instance than it is across the dataset the model has been trained on (or datasets from all tasks) \ta{Do saliency scores correlate with TF-IDF?}
    \item Relation between human and machine salience (if annotator rationales, i.e. binary human-labeled ground truth salience scores, are present): $x$ unexpectedly is the most salient word. / Contrary to human annotation, $x$ is not salient. \ta{How sure were human annotators about labels? Confidence scores of model vs. human?}
\end{itemize}

==> tables/tab_examples.tex <==
\begin{table}[ht!]
\begin{tabular}{l|p{5cm}}
Dialogue Act & Example \\
\hline
Inform &  \textit{I'm in 507. I have a few problems with my room.} \\
Question & \textit{Good morning, sir. Is there a bank near here?} \\
Directive & \textit{Good. Let's go now.} \\
Commissive & \textit{Really? I hope I can have a chance to taste it.} \\
\end{tabular}
\caption{\data{DailyDialog} dialogue act examples}
\label{tab:daily-dialog-examples}
\end{table}

==> tables/tab_rank_corr.tex <==
\begin{table}[t!]
    \centering

    %\resizebox{\columnwidth}{!}{%
        \begin{tabular}{r|ccc}

        \toprule
        Datasets & \textbf{C}orr. & \textbf{H}elp. & \textbf{S}at.\\

        \midrule
        \data{BoolQ} & 0.97 & 0.91 & 0.91 \\
        \data{OLID} & 0.87 & 0.94 & 0.90 \\
        \data{DailyDialog} & 0.90 & 0.91 & 0.94 \\
        
        \bottomrule
        \end{tabular}
    %}
    \caption{Kendall's $W$ rank correlation coefficient between \textbf{C}orrectness, \textbf{H}elpfulness and \textbf{S}atisfaction ratings on our three datasets as reported in Table~\ref{tab:singleratings}.
    }
    \label{tab:rank_corr}
\end{table}
